Multi-parameter optimization of attenuation data for characterizing grain size distributions and application to bimodal microstructures

In this paper, the effect on the ultrasonic attenuation of the grain size heterogeneity in polycrystals is analyzed. First, new analytical developments allowing the extension of the unified theory of Stanke and Kino to general grain size distributions are presented. It is then shown that one can additively decompose the attenuation coefficient provided that groups of grains are defined. Second, the study is specialized to a bimodal distribution of the grain size for which microstructures are numerically modeled by means of the software Neper. The additive partition of the attenuation coefficient into contributions coming from large and small grains motivates the derivation of an optimization procedure for characterizing the grain size distribution. The aforementioned approach, which is based on a least squares minimization, is at last presented and illustrated on both analytical and numerical attenuation data. It is thus shown that the method provides satisfying approximations of volume fractions of large grains and modal equivalent diameters from the frequency-dependent attenuation coefficient.

==> numerical_procedure.tex <==

\subsection{Properties of the continuum problems}

% Change results by those taking into account W
% Check whether it is possible to get a master curve for bimodal microstructures
%% => Can one use this to deduce the presence of a bimodal distribution? Apparently it is not possible

% Change plan: theory - microstructures considered (2D; 3D) - procedure (2D; 3D) based on a data base - numerical evidences (2D) based on a data base?

% 3D monomodal microstructures are being created so that the procedure can be used with alpha_W^3D

\begin{figure}[ht]
  \centering
  \input{pgfFigures/geometry2D}
  \caption{Geometry and loading conditions of the considered problem}
  \label{fig:problem_setting}
\end{figure}

A sum of two Ricker signals varying in time with frequency content centered to $5$MHz and $10$MHz.
For such an external loading, the valid frequency domain is limited to a range $4$--$16$MHz, which leads to a range from $375\mu$m to $1.5$mm for wavelengths.
Hence, the Rayleigh region and the Rayleigh-to-stochastic transition domain are covered with respect to the considered grain sizes.

\subsection{Discretization}

DG method first order, time step, structured mesh with size satisfying the convergence properties shown in [van Pamel, Xue] regarding the wave length etc.
\review{Il faudra dire a un moment qu'on fait du maillage carre}

\subsection{Post-treatment of the ultrasonic data}

The velocity solution provided by the Finite Element procedure in time domain is recorded at $N^{\text{points}}$ lying on the free end of the sample.
Those signals are then windowed in order to extract at each point the reflection of the incident wave only.
In order to take into account the dispersion resulting form the constitutive heterogeneities, the time window is defined for one point as: $t\in \[T_{v_{max}}-T_r/2,\: T_{v_{max}}+T_r/2\]$, where $T_{v_{max}}$ is the time of maximum velocity at that point.
The averaged of the field computed on the free end is next transformed in the frequency domain for the homogeneous reference solid and the heterogeneous sample.
At last, the attenuation coefficient is computed as:
\begin{equation}
  \label{eq:numerical_alpha}
  \alpha(f) = \frac{1}{2 D}\log\(\frac{\abs{v^{Iso}(f)}^2}{\abs{v^{Sample}(f)}^2}\)
\end{equation}
where $D\equiv l$ is the propagation distance.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "manuscript"
%%% End:


==> tabular/2D_optimization_Voigt.tex <==

\begin{tabular}{ccc|cc|cccc}
  \multicolumn{3}{c|}{Input parameters} & \multicolumn{2}{c|}{Monomodal fitting} & \multicolumn{4}{c}{Bimodal fitting}\\
  $F_{LG}$ (\%)& $d^{SG}$ & $d^{LG}$ & $d_{opt}$ & $\epsilon_{Mono}$ (\%) &  $F^{opt}_{LG}$ (\%)& $d_{opt}^{SG}$ & $d^{LG}_{opt}$& $\epsilon_{Bi}$ (\%) \\
  \hline
  % 25 & 160 & 240 & 178 & 2 & 44 & 151 & 210 & $4\times 10^{-2}$\\
  % 50 & 160 & 240 & 199 & 2 & 68 & 148 & 221 & $6\times 10^{-2}$\\
  % 75 & 160 & 240 & 221 & 1 & 90 & 134 & 229 & $5\times 10^{-2}$\\
  25 & 160 & 240 & 176 & 2.4 & 38 & 154 & 224 & $9.8\times 10^{-2}$\\
  50 & 160 & 240 & 194 & 3.5 & 61 & 153 & 230 & $5.8\times 10^{-2}$\\
  75 & 160 & 240 & 215 & 2.5 & 95 & 99 & 224 & $2.1\times 10^{-1}$\\
  \hline
  % 25 & 80 & 240 & 83 & 14 & 29 & 80 & 240 & $1$\\
  % 50 & 80 & 240 & 91 & 24 & 56 & 80 & 240 & $1$\\
  % 75 & 80 & 240 & 229 & 9 &  81 &80  &240  & $1 $\\
  25 & 80 & 240 & 116 & 12 & 30 & 80 & 239 & $2.2\times 10^{-1}$\\
  50 & 80 & 240 & 158 & 15 & 58 & 80 & 236 & $4.4\times 10^{-1}$\\
  75 & 80 & 240 & 200 & 10 & 82 & 80 & 233 & $3.5\times 10^{-1}$\\

  \hline
  % 25 & 80 & 160 & 89 & 5 & 27 & 80 & 160 & $2\times 10^{-1}$\\
  % 50 & 80 & 160 & 104 & 8 & 54 & 80 & 157 & $2\times 10^{-1}$\\
  % 75 & 80 & 160 & 145 & 6 & 79 & 80 & 157 & $2\times 10^{-1}$\\
  25 & 80 & 160 & 100 & 4.3 & 29 & 80 & 155 & $1.6\times 10^{-1}$\\
  50 & 80 & 160 & 122 & 5.2  & 55 & 80 & 155 & $1.5\times 10^{-1}$\\
  75 & 80 & 160 & 142 & 2.9  & 82 & 80 & 155 & $1.4\times 10^{-1}$\\
  \hline
  35 & 90 & 190 & 127 & 6.1 & 31 & 98 & 208 & $4.4\times 10^{-1}$
\end{tabular}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../manuscript"
%%% End:


==> tabular/3D_optimization_Voigt.tex <==

\begin{tabular}{ccc|cc|cccc}
  \multicolumn{3}{c|}{Input parameters} & \multicolumn{2}{c|}{Monomodal fitting} & \multicolumn{4}{c}{Bimodal fitting}\\
  $F_{LG}$ (\%)& $d^{SG}$ & $d^{LG}$ & $d_{opt}$ & $\epsilon_{Mono}$ (\%) &  $F^{opt}_{LG}$ (\%)& $d_{opt}^{SG}$ & $d^{LG}_{opt}$& $\epsilon_{Bi}$ (\%) \\
  \hline
  % 25 & 160 & 240 & 176 & 3.4 & 21 & 162 & 240 & $4\times 10^{-2}$\\
  % 50 & 160 & 240 & 204 & 5.1 & 47 & 161 & 240 & $8\times 10^{-2}$\\
  % 75 & 160 & 240 & 226 & 3.4 & 74 & 164 & 240 & $6\times 10^{-2}$\\
  25 & 160 & 240 & 177 & 1.9 & 26 & 159 & 238 & $2.1\times 10^{-2}$\\
  50 & 160 & 240 & 195 & 3.6 & 54 & 156 & 240 & $7.9\times 10^{-2}$\\
  75 & 160 & 240 & 215 & 3.6 & 77 & 158 & 240 & $2.0\times 10^{-2}$\\
  \hline
  % 25 & 80 & 240 & 90 & 25 & 28 & 80 & 235 & $0.3$\\
  % 50 & 80 & 240 & 100 & 37 & 53 & 81 & 239 & $0.3$\\
  % 75 & 80 & 240 & 126 & 37 & 72 & 88 & 240 & $0.3$\\
  25 & 80 & 240 & 108 & 13 & 29 & 80 & 236 & $4.9\times 10^{-2}$\\
  50 & 80 & 240 & 162 & 15 & 54 & 80 & 237 & $1.4\times 10^{-1}$\\
  75 & 80 & 240 & 195 & 13 & 76 & 80 & 240 & $3.0\times 10^{-1}$\\

  \hline
  25 & 80 & 160 & 95 & 4.4 & 28 & 80 & 159 & $1.3\times 10^{-2}$\\
  50 & 80 & 160 & 117 & 6.3 & 54 & 80 & 159 & $3.2\times 10^{-2}$\\
  75 & 80 & 160 & 143 & 3.8 & 71 & 90 & 164 & $1.1\times 10^{-1}$\\
  \hline
  35 & 90 & 190 & 122 & 7.5 & 42 & 87  & 183 & $1.7\times 10^{-2}$
\end{tabular}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../manuscript"
%%% End:


==> tabular/diameters_bimodalFitting.tex <==
% \begin{tabular}{l|ccc|ccc|ccc}
%   FLG & \multicolumn{3}{c|}{ $240$--$160 \mu$m} &\multicolumn{3}{c|}{$240$--$80 \mu$m} &\multicolumn{3}{c}{$160$--$80 \mu$m} \\
%    & FLG$^{opt}$ & $\bar{d}_{small}^{opt}$ ($\mu$m) & $\bar{d}_{large} ^{opt}$ ($\mu$m) & FLG$^{opt}$ & $d_{small}^{opt}$ ($\mu$m) & $\bar{d}_{large} ^{opt}$ ($\mu$m) & FLG$^{opt}$ & $d_{small}^{opt}$ ($\mu$m) & $\bar{d}_{large} ^{opt}$ ($\mu$m)  \\
%   \hline
%   10 \% & 9 & 160 & 240 &  9 &  80 &240 & 9& 80&160\\  
%   25 \% & 25 & 159 & 239 & 25 & 79  &239& 24& 80&160\\  
%   40 \% & 39 & 160 & 240 & 39 & 80 & 240& 40& 79&160\\  
%   50 \% & 50 & 159 & 239& 50&  79&  239& 50& 79&159\\  
%   60 \% & 60 & 159 & 239& 59& 80 & 240 &59& 80&160\\  
%   75 \% & 74 & 160 & 240& 74& 80 & 240 &74& 80&160\\  
%   90 \% & 90 & 159 & 240& 70& 79 & 139 &89& 80 &160
% \end{tabular}

\begin{tabular}{l|ccc}
  $F_{LG}$ &   $F_{LG}^{opt}$ ($\%$) & $d_{small}^{opt}$ ($\mu$m) & $\bar{d}_{large} ^{opt}$ ($\mu$m)  \\
  \hline
  10 \% &  9 &  80 &240 \\  
  25 \% & 25 & 79  &239\\  
  40 \% & 39 & 80 & 240\\  
  50 \% & 50&  79&  239\\  
  60 \% & 59& 80 & 240 \\  
  75 \% & 74& 80 & 240 \\  
  90 \% & 90& 79 & 139 
\end{tabular}


==> tabular/diameters_monomodalFitting.tex <==
% \begin{tabular}{l|cc|cc|cc}
%   FLG & \multicolumn{2}{c|}{ $240$--$160 \mu$m} &\multicolumn{2}{c|}{$240$--$80 \mu$m} &\multicolumn{2}{c}{$160$--$80 \mu$m} \\
%    & $d^{opt}$($\mu$m) & $\bar{d}$($\mu$m) &$d^{opt}$($\mu$m) & $\bar{d}$($\mu$m) &$d^{opt}$($\mu$m) & $\bar{d}$($\mu$m) \\
%   \hline
%   10 \% & 166 & 168 & 81 & 96 &  82 & 88\\  
%   25 \% & 176 & 180 & 84 & 120&  87 & 100\\  
%   40 \% & 187 & 192 & 89 & 144&  94 & 112\\  
%   50 \% & 195 & 200 & 169& 160& 103 & 120 \\  
%   60 \% & 203 & 208 & 194& 176& 117 & 128\\  
%   75 \% & 216 & 220 & 216& 200& 140 & 140\\  
%   90 \% & 230 & 232 & 232& 224& 153 & 152
% \end{tabular}
\begin{tabular}{l|cc}
  $F_{LG}$   &$d^{opt}$($\mu$m) & $\bar{d}$($\mu$m)  \\
  \hline
  10 \%  & 81 & 96 \\  
  25 \%  & 84 & 120\\  
  40 \%  & 89 & 144\\  
  50 \%  & 169& 160 \\  
  60 \%  & 194& 176\\  
  75 \%  & 216& 200\\  
  90 \%  & 232& 224
\end{tabular}

